Counterfactual States for Atari Agents via Generative Deep Learning

Although deep reinforcement learning agents have produced impressive results in many domains, their decision making is difficult to explain to humans. To address this problem, past work has mainly focused on explaining why an action was chosen in a given state. A different type of explanation that is useful is a counterfactual, which deals with "what if?" scenarios. In this work, we introduce the concept of a counterfactual state to help humans gain a better understanding of what would need to change (minimally) in an Atari game image for the agent to choose a different action. We introduce a novel method to create counterfactual states from a generative deep learning architecture. In addition, we evaluate the effectiveness of counterfactual states on human participants who are not machine learning experts. Our user study results suggest that our generated counterfactual states are useful in helping non-expert participants gain a better understanding of an agent's decision making process.

==> experiments_with_study1.tex <==
%things to include for results:
% 1) Images from 3 Atari games
% 2) User study results
%     i) Realism results
%     ii) # of participants with decrease/no change/increase in rating for understanding agent
%     ii) Noinsight count histogram (1-10) and the # of users in each bin
%     iii) Number of participants with noinsight for each counterfactual % example
%     


\subsection{Experimental Setup}
% lwneal suggestion
The pre-trained agent is a deep convolutional network trained with Asynchronous Advantage Actor-Critic (A3C) to maximize score in an Atari game. Games are played with a fixed frame-skip of 8 (7 for Space Invaders). We decompose the agent into two functions: $A(\bm{s})$ which takes as input 4 concatenated video frames and produces a 256-dimensional vector $\bm{z}$, and $\bm{\pi}(z)$ which outputs a distribution among actions. To generate the dataset $\mathcal{X}$, we set $\epsilon$ exploration value to $0.2$.  %The A3C agent's value function approximation is discarded.
% maybe \cite{pmlr-v80-greydanus18a} here
%For our pre-trained agent, we take a traditional A3C agent with 4 frames concatenated as a state input. We use the Atari Learning Environment to play 3 different games. The games are played with a frameskip of 8 (7 for Space Invaders). The agent is a deep convolutional neural network that creates a 256-dimensional representation $z$ of the input frames, which then approximates the long term value of the state along with the probability of taking each action.

The encoder $E$ consists of 6 convolutional layers followed by 2 fully-connected layers with LeakyReLU activations and batch normalization. The output $E(\bm{s})$ is a 16-dimensional vector. We find a value of $\lambda=20$ enforces a good tradeoff between state reconstruction and reliance on $\bm{\pi}(z)$. 
%The Encoder is a deep neural network with 6 convolution layers followed by 2 fully connected layers. For our experiments, the output of the encoder is a 16-dimensional vector. For setting the hyper parameter $\lambda$, we find a value of 20 is sufficient for adequate reconstruction of the states and for forcing the generator to rely on the input $\bm{\pi}(z)$.
% lwneal suggestion
The generator $G$ consists of one fully-connected layer followed by 6 transposed convolutional layers, all with ReLU activations and batch normalization.
%The Generator is a deep neural network with a fully connected layer and 6 transposed convolutional layers. 
% lwneal suggestion
The encoded state $E(\bm{s})$ and the action distribution $\bm{\pi}(\bm{z})$ are fed to the first layer of the generator, and additionally $\bm{\pi}(\bm{z})$ is appended as an additional input channel to each subsequent layer.
%To provide the generator with the agent's policy, we append $\bm{\pi}(z)$ to each layer given as input to the generator. For this purpose, $\bm{\pi}(z)$ is the concatenation of the probabilities [0, 1] for taking each action at the given state. We append this as an additional constant input channels for all the convolutions of the generator. 
% lwneal suggestion
The discriminator $D$ consists of two fully-connected layers followed by a softmax function, and outputs a distribution among actions with the same dimensionality as $\bm{\pi}(\bm{z})$.
%The discriminator is a network with 2 fully connected layers of size 16 followed by a soft-max layers the same size as the game environment action space.
% lwneal suggestion
The Wasserstein encoder $E_w$ consists of 3 fully-connected layers mapping $\bm{z}$ to a 128-dimensional vector $\bm{z}_w$.%, normalized such that $||z_w||_w = 1$.
The corresponding Wasserstein decoder $D_w$ is symmetric to $E_w$ and maps $\bm{z}_w$ back to $\bm{z}$.
%The Wasserstein encoder is a 3 layer fully connected network, which outputs a 128-dimensional vector $z_w$ normalized such that $||z_w||_2 = 1$. The Wasserstein decoder is symmetric to the encoder.

All models are constructed and trained using PyTorch \cite{paszke2017automatic}.
For more information about our architecture and training parameters, our code and supplementary material can be accessed at: \url{https://github.com/cf-anonymous/cf-anonymous}


%\hl{For more details please see this supplementary material: hyperlink}


\subsection{Baseline Comparisons}

\begin{figure}[t]
    \centering
    \includegraphics[width=.32\linewidth]{ablation_only_agent_latent_cf.png} 
    \includegraphics[width=.32\linewidth]{bw_frame23_kappa5_Orig4_Adv5_Delta2.png} 
    \includegraphics[width=.32\linewidth]{bw_frame127_kappa5_Orig5_Adv4_Delta3.png} %
    %\caption{Applying CEM to generate counterfactuals via pertinent negatives for Space Invaders. The publicly-available CEM source utilizes the input to the neural network, which are greyscale atari frames. }
    \caption{Counterfactual states generated using the ablated model (\textbf{Left}), and CEM with two choices of parameters on different states (\textbf{Middle} and \textbf{Right}).}
    
    \label{fig:CEM}%
\end{figure}

We compare our full method against an ablated version trained without adversarial loss, and against the Contrastive Explanation Method (CEM) \cite{Dhurandhar18}.

In the ablated version of the network, the encoder, discriminator, and Wasserstein autoencoder are removed, and the generator is trained with MSE loss to reconstruct $\bm{s}$ given $\bm{z}$ as input.
Counterfactual images are generated by performing gradient descent with respect to $\bm{z}$ to maximize $\bm{\pi}(\bm{z},a')$ for a counterfactual action $a'$.
We find that counterfactual states generated in this way fail to construct a fully realistic state as shown in Figure \ref{fig:CEM} (left).
Other ablations of the network architecture generated poor counterfactual states, indicating that all components of our architecture are necessary. These results can be found in our supplementary material.


%In order to investigate the quality of our counterfactual states generation method, we compare against other methods.
%Here we highlight an interesting ablation example and the Contrastive Explanation Method.
%For an extensive analysis of all our ablations, please see our \hl{supplementary material}.
%For this ablation, we train our generator with MSE on only the agent's learned latent representation $z$.
%The image is created by performing gradient descent on the latent point $z$ to maximize the probability of an action $a'$, which is then passed into the generator. 
%The other ablations had one of two problems: First, the counterfactual states looked identical to the reconstructed state.
%Second, the reconstructed states did not accurately reconstruct the original input state, meaning the counterfactual state would be a moot point.

\label{sec:CEM}
The Contrastive Explanation Method (CEM) can generate \textit{pertinent negatives} which highlight which absent features would cause the agent to select an alternate action.
We generate pertinent negatives from Atari states with pixels as features, and interpret them as counterfactual states.

We performed an extensive search over hyper-parameters to generate realistic states, but found CEM very difficult to tune for this high-dimensional space. The generated counterfactual states were either identical to the original query state or they had excessive ``snow'' artifacts as shown in Figure \ref{fig:CEM} (middle and right).

%We compare our method to CEM on the task of producing counterfactual states.
%CEM's method for generating pertinent negatives can be readily modified to produce counterfactuals that highlight which absent features would most cause the agent to select an alternate action.
%Figure \ref{fig:CEM} shows the results. One of the main difficulties in applying CEM to Atari images is the tuning of hyperparameters over this high dimensional space.
%We performed an extensive search over hyper-parameters to find reasonable images, but found that either the counterfactual states were identical to the original query state or they had excessive ``snow'' artifacts. 

\subsection{Example Counterfactual States}


%\begin{figure*}[t]
    %\centering
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_space_ex1.png} 
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_space_ex2.png} 
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_space_ex3.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_qbert_a_upright_cf_upleft.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_qbert_actionUP_cfDOWN.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_seaquest_ex1.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_seaquest_ex2.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/orig_seaquest_ex3.png}
    %\caption{Space invaders original actions: ``move right''..... Qbert: ``Move up-right''.... Seaquest: move up and fire, move left and fire, move up left and fire}
%\end{figure*}

\begin{figure*}[t]
    \centering
    %\includegraphics[width=.137\linewidth]{cf_imgs/cf_space_ex1.png} 
    %\includegraphics[width=.137\linewidth]{cf_imgs/cf_space_ex2.png} 
    %\includegraphics[width=.137\linewidth]{cf_imgs/cf_space_ex3.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/cf_qbert_a_upright_cf_upleft.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/cf_qbert_actionUP_cfDOWN.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/cf_seaquest_ex1.png}
    %\includegraphics[width=.137\linewidth]{cf_imgs/cf_seaquest_ex2.png}
    %\includegraphics[width=\linewidth]{cf_imgs/counterfactual_games.png}
 \includegraphics[width=\linewidth]{cf_imgs/counterfactual_games_with_boxes.png}
    \caption{Example query state (left) and counterfactual state (right) pairs.
    \textbf{Top-Left}: Space Invaders, $a =$ \textit{MoveRight}, $a'=$ \textit{Fire}.
    \textbf{Bottom-Left}: $a =$ \textit{MoveRight}, $a'=$ \textit{MoveLeft}.
    \textbf{Top-Center}: Qbert, $a=$ \textit{MoveUpRight}, $a'=$ \textit{MoveDownLeft}.
    \textbf{Bottom-Center}: $a=$ \textit{MoveUpRight}, $a'=$ \textit{MoveUpLeft}.
    \textbf{Top-Right:} Seaquest, $a=$ \textit{MoveUpAndRight}, $a'=$ \textit{MoveUpLeftAndFire}.
    \textbf{Bottom-Right:} $a=$ \textit{MoveLeftAndFire}, $a'=$ \textit{MoveDown}. }
    %\caption{Space invaders cf actions:fire, and move left..... Qbert: move upleft and move down left.... Seaquest: ``Move up-left and fire'', ``Move down'', ``Move up-left''}
    \label{fig:cf_imgs}%
\end{figure*}


% lwneal suggestion:
% The following figures demonstrate counterfactual state generation for various A3C agents. In each figure, the leftmost image is the original state $s$, and the right image is the counterfactual state $s'$, altered from $s$ so that the agent will take action $a'$. The center image highlights in red the absolute pixel-wise difference between $s$ and $s'$.
We now show examples of counterfactual states for pre-trained agents in various Atari games. In Figure \ref{fig:cf_imgs}, we show pairs of images where the 
the left image is the original query state where the agent would take action $a$ according to its policy, and the right image is the counterfactual state where the agent would take the selected action $a'$. 

%Hey check out our examples. 

\paragraph{Space Invaders}
% lwneal suggestion
In this game, an agent exchanges fire with approaching enemies while taking cover underneath three barriers. The examples in Figure \ref{fig:cf_imgs} reveal that the agent has learned to prefer specific locations for safely lining up shots. %to fire only when its line of sight is not blocked by a barrier. % and maybe also some additional insights here? what did the counterfactuals teach us about the agent?
%In the game of Space Invaders, you are tasked with shooting approaching aliens while avoiding their shots. We see from these counterfactual states that the agent knows about barriers, and that they blocks shots from both above and below.
%the agent has learned preffered locations: linining up shots to enemies and utilizing barriers


%\begin{center}
%    \includegraphics[width=\columnwidth]{space_ex1.png}
%    $a = \text{``Move right''}$. \  $a' = \text{``Fire''}$
%    \includegraphics[width=\columnwidth]{space_ex2.png}
%    $a = \text{``Move left and fire''}$. \  $a' = \text{``Move right and fire''}$
%    \includegraphics[width=\columnwidth]{space_ex3.png}
%    $a = \text{``Move right''}$. \  $a' = \text{``Move left''}$
%\end{center}





% you this image? clearly the AI knows about barriers
% check out this other one, the AI has preference for shooting lower enemies

\paragraph{$\text{Q}^*$bert}
% lwneal suggestion:
% In $\text{Q}^*$bert, an agent must visit each tile while avoiding enemies. The counterfactual states show that the agent has learned to traverse the tiles in a particular pattern. This policy achieves a high score, but may not generalize well.
In this game, an agent's goal is to jump on uncolored squares and avoid enemies.
In Figure \ref{fig:cf_imgs} (top-center), the agent will jump down and left if the Qbert character had been higher up on the structure. In Figure \ref{fig:cf_imgs} (bottom-center), the counterfactual shows that the up-right square is yellow (already visited), which will cause Qbert to move up-left.
%)chooses to take a different path through the structure because of if an uncolored square had previously been landed on.


%Here you can see the AI is about to land on a square and take the jump upright action.
%We ask the AI what would need to change to jump upleft instead of upright and here's what is says

%\begin{center}
%    \includegraphics[width=\columnwidth]{qbert_a_upright_cf_upleft.png}
%    $a = \text{``Move up-right''}$ \  $a' = \text{``Move up-left''}$
%
%     \includegraphics[width=\columnwidth]{qbert_actionUP_cfDOWN.png}
%     $a = \text{``Move up-left''}$ \  $a' \text{``Move down-left''}$
%
%\end{center}

\paragraph{Seaquest}
In this game, an agent must shoot incoming enemies while rescuing friendly divers. 
Figure \ref{fig:cf_imgs} (top-right) shows that a new enemy must appear to the left in order for the agent to take an action that turns the submarine around while firing. Thus, the agent has an understanding about enemy spawns and submarine direction.
Figure \ref{fig:cf_imgs} (bottom-right) shows an unrealistic counterfactual with two submarines.


%\begin{center}
%    \includegraphics[width=\columnwidth]{seaquest_ex1.png}
%    $a = \text{``Move up and fire''}$ \ $a' = \text{``Move up-left and fire''}$
%    \includegraphics[width=\columnwidth]{seaquest_ex2.png}
%    $a = \text{``Move left and fire''}$ \ $a' = \text{``Move down''}$
%    \includegraphics[width=\columnwidth]{seaquest_ex3.png}
%    $a = \text{``Move up-left and fire''}$ \ $a' = \text{``Move up-left''}$
%\end{center}

\subsection{User Study}
Evaluating counterfactual states is a challenging problem. ``Good'' counterfactual states provide insight to a human as to why the agent performed a certain action. This criterion is difficult to capture through quantitative metrics, which often measure the wrong thing. For instance, using the probability $\pi(\bm{s'},a')$ as a metric for a counterfactual state $\bm{s}'$ is misleading because this probability can be swayed by Atari images that are obvious unrealistic to humans or by adversarial examples with imperceptible changes to the original state $\bm{s}$.

As a result, we evaluate our counterfactual states through a user study with participants who were not experts in machine learning. Participants played Space Invaders and then were given a tutorial to explain counterfactual states. 
In the first part of the study, participants rated the realism of randomly ordered game images on a Likert scale from 1 to 6 (higher is more realistic). 
The images were a mix of images generated by three different sources: the actual game, our counterfactual method, and our ablation experiment. 

In the second part, we showed the users 10 counterfactual states displayed alongside the original query state and an image that highlights the changes. We chose the game images from a replay of an existing game. 
The specific images, serving as query states for our counterfactuals, were chosen using a heuristic based on entropy, which has been used in the past for choosing key frames for establishing trust \cite{huang2018}. 
For diversity, if a key frame was selected, we do not allow images from the next two time-steps to be selected. 
Once a query state was selected, we selected the counterfactual action as the one that required the largest $L_2$ change between the original latent state $\bm{z}$ and the counterfactual latent state $\bm{z'}$ (ignoring the no-operation action). 
We emphasize that the counterfactual states were not hand-picked; rather, they were selected by ranking game images according to our heuristic and then selecting the counterfactual action according to the previous criterion.
For each counterfactual state generated, we asked the participant what they learned about the agent's decision making, and they answered in a free text response box. For additional details about the user study, please see our supplementary material.
 
\paragraph{Study Results} In terms of realism, the average ratings on the 6 point Likert scale were 1.93 (ablation), 4.00 (counterfactual states) and 4.97 (actual game). The differences between the realism ratings for the counterfactual states and real states were not statistically significant at $\alpha=0.05$ (p-value=0.458, one-sided Wilcoxon signed-rank test). These results show that our counterfactual states were on average close to appearing realistic, but there were some flaws. 

For their free text responses, we developed a qualitative code set based on 6 codes corresponding to elements of the game: Death, Barrier, Enemies, Pose, Shot, and NoInsight (NI). These codes were developed after two independent coders reached a score above 0.8 with Cohen's Kappa on 20\% of the data. The {\it NoInsight} code indicates that the participant gained no insight from the counterfactual state. This code was determined from the free text response by the participant saying they learned nothing, restating the obvious, transcribing the counterfactual image, or saying something invalid. In contrast, the other codes correspond to the participant learning something about the agent's behavior due to its awareness of various aspects of the game. The validity of the majority of these responses is fairly straightforward to assess in Space Invaders due to the simplicity of the game. 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{histogram.png}
    \caption{A histogram of the number of \textit{NI} codes per participant.}
    %\caption{A histogram showing the number of \textit{NoInsight} codes per participant.}
    \label{fig:histogram}
\end{figure}


%%%%%%%%%%%%%%
\iffalse
\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
 & \multicolumn{8}{|c|}{\# NoInsight codes assigned}\\ \hline
 & 0 & 1 & 2 & 3 & 4 & 5 & 6 & $ \geq 7$\\ \hline
\# Participants  & 4 & 8 & 5 & 4 & 2 & 5 & 2 & 0\\ \hline
\end{tabular}
%\caption{The number of participants that were assigned 0, 1, 2... NI codes.}
\caption{Histogram of \textit{NoInsight} codes per participant}
\label{table:histogram}
\end{table}
\fi
%%%%%%%%%%%%%%%%%

Figure \ref{fig:histogram} is a histogram of the number of participants whose free-text answers were coded as NoInsight. 
We see that the typical participant gained some form of insight for the majority of counterfactual explanations. 
Approximately 17/30 participants found two or fewer counterfactual states to be non-informative and these non-informative examples varied among participants. 
Even for the 7 users who found 5 or 6 of the counterfactuals not insightful, they were still able to glean something out of the remaining counterfactual explanations. 

% 2) User study results
%     i) Realism results
%     ii) # of participants with decrease/no change/increase in rating for understanding agent
%     ii) Noinsight count histogram (1-10) and the # of users in each bin
%     iii) Number of participants with noinsight for each counterfactual % example
%     


For all 10 counterfactual states in our user study, no single image was uninformative to all participants. 
Table \ref{table:codesbyexample} breaks down the number of codes assigned to each counterfactual example. 
Example 8 seemed to be the most informative as only 3/30 participants were assigned the NoInsight code. 
For the worst counterfactual states, namely Examples 2 and 9, 40\% of participants gained no insight from a counterfactual state but the remaining 60\% of users were able to learn something about the agent. Images of all 10 counterfactual states are shown in the supplementary material. 
In light of the fact that some counterfactual states in our study were not completely realistic because they did not represent a valid game state, this result shows that nevertheless, some participants were still able to learn something about the agent from them.


\begin{table}[t]
\centering
\begin{tabular}{|l||l|l|l|l|l|l|} 
\hline
Ex & Death & Barrier & Enemies & Pose & Shot & NI \\ \hline \hline
1  & 0     & 8       & 1       & 10   & 4    & 7   \\ \hline
2  & 0     & 2       & 10      & 6    & 0    & 12  \\ \hline
3  & 2     & 13      & 3       & 1    & 5    & 6   \\ \hline
4  & 0     & 17      & 1       & 3    & 2    & 7   \\ \hline
5  & 0     & 11      & 6       & 8    & 0    & 5   \\ \hline
6  & 0     & 7       & 16      & 2    & 0    & 5   \\ \hline
7  & 0     & 3       & 7       & 10   & 1    & 9   \\ \hline
8  & 0     & 1       & 16      & 3    & 7    & 3   \\ \hline
9  & 0     & 3       & 12      & 1    & 2    & 12  \\ \hline
10 & 0     & 0       & 14      & 5    & 2    & 9    \\
\hline
\end{tabular}
\caption{A breakdown of the number of codes assigned to each counterfactual state example showed to participants}
\label{table:codesbyexample}
\end{table}

The results from Figure \ref{fig:histogram} and Table \ref{table:codesbyexample} indicate that the counterfactual states are indeed useful but in different ways to different participants. 
Taken together, these results suggest that counterfactuals change users' mental models of how these RL agents work in different ways; this is an interesting topic to investigate more deeply in the future.

We also asked the participants to rate their understanding of the agent on a 6 point Likert scale before and after seeing the counterfactual states. 
We found 15 users' understanding increased, 8 decreased, and 7 stayed the same (p-value = 0.098, one-sided Wilcoxon signed-rank test).  
These results are close to being statistical significant at the $\alpha=0.05$ level and they suggest that counterfactual states are indeed providing most users with enough insight into an agent's decision making to improve their understanding of how they work.


==> methodology_old.tex <==
\subsection{Trained RL Agent}
We assume that a trained deep reinforcement learning agent is provided for diagnosis. In our work, we train RL agents using the A3C algorithm \cite{mnih2016}, which learns a policy distribution $\pi(s)$ and a value function estimate $V^{\pi}$. 

Atari agents are trained on images and have the same recurrent architecture. The input at each time step is a preprocessed version of the current frame.
The input is processed by 4 convolutional layers (each with 32 filters, kernel sizes of 3, strides of 2, and paddings of 1), a single fully connected layer with 256 hidden units, and lastly two parallel fully-connected layers.
The first of the parallel fully-connected layers provides the policy function $\pi(s)$, via a softmax distribution among the $n$ possible actions possible at any time step in the game.
The second is trained to approximate the value function $V(s)$. 

\subsection{Auto-Encoder Architecture}
%The input, as shown in fig 1, is processed by 5 convolution layers (increasing number of kernels from 64 to 512, alternating kernel sizes of 3 and 4, with strides of 1 and 2 respectively, and padding of 1) and a fully connected layer to create a latent point z.

We extend the work of \citet{lample2017fader}; where they create a disentangled latent space by training an auto-encoder that attempts to remove labels from the encoded inputs. And they train a discriminator, along with the encoder, to ensure label information is removed from the latent space.

We propose a disentangled auto encoding model to recreate reinforcement learning states. The model consists of four parts: The Agent $A(s)$, which maps from Atari frames states $s$ to a policy $\pi$ and a value estimation $V(s)$, but also has its own latent representation $z_A$. The Encoder $E(s)$, which also maps Atari frames $s$ to a separate latent space $z_E$ that has information about $A(s)$ removed. The Discriminator $D(z_E)$ takes as input the Encoder's latent representation and predicts $\pi$. Lastly, the Generator $G(z)$, reconstructs the input Atari frames from the concatenated latent points $z = z_E;z_A$.

The loss of the discriminator is the Kullback-Leibler Divergance from the output probability of the agent $A$ taking an action $a$ in state $s$.

\begin{equation}
\mathbf{KL(D||\pi)} = \sum_{s \in \mathbf{S}} \sum_{a \in \mathbf{A}} P(a|\pi(A(s))) * log \dfrac{P(a|\pi(A(s)))}{P(a|D(E(s)))} 
\end{equation}

%\begin{equation}
%KL({Q}\|{P}) = E_{f\sim{Q}}\log{\frac{{Q}(f)}{{P}(f)}}
%\end{equation}

The loss of the Encoder and Generator is defined in two parts: the pixel-wise reconstructions of all visited game states S and the adversarial loss of the discriminator, with a weighting term, $\lambda$, to control the effect of the discriminator.

%We start with a simple auto encoding model that recreates the input Atari preprocessed frame. The model consists of two parts: The Encoder $E(s)$, which maps from Atari frame stats s, to a latent space and a generator $G(z)$, which maps from latent points back to Atari frames.  The Generator takes, as input, a latent point and processes it through 5 layers of deconvolution. Every layer, but the last, is followed by a rectified linear function.


\begin{equation}
\mathbf{L_{E,G}} = - \lambda_E \mathbf{KL(D||\pi) + \sum_{s \in \mathbf{S}} ||s - G(E(s);A(s))||_2^2 }
\end{equation}


%TODO: make a table
%In an effort to further improve image reconstructions, the output of the trained agent, $\pi(s)$ is concatenated with the latent point z. The output of this agent is the probability mass function for the probability of taking each discrete action, where the highest probability action is taken. The agent takes as input the Atari state s. This transforms our overall architecture from $G(E(s))$ to $G([E(s);\pi(s)])$. We can see an improvement by using this architecture through the average reconstruction loss. See Fig. 1 for a specific example. 

%\begin{figure}
%\begin{center}
%    \includegraphics[width=\linewidth]{disentangled_example.png}
%\end{center}
%\caption{Example of the difference between simple auto-encoding and disentangling variables in the latent space for the auto-encoder. The two bullets from the original frame are reconstructed better through the disentangled representation.}
%\end{figure}


\begin{figure*}
\begin{center}
    \includegraphics[width=\linewidth]{architecture_pic.png}
\end{center}
\caption{The overall network architecture.}
\end{figure*}


\subsection{Counterfactual Image Generation}


We will refer to (Lawrence et. al, 2018) for their explanation of counterfactuals. 

In logic, a conditional statement $p \rightarrow q$ is true if the antecedent statement $p$ implies the consequent $q$.
A counterfactual conditional, $p \counterfactual q$ is a conditional statement in which $p$ is known to be false \cite{lewis2013counterfactuals}.
It can be interpreted as a \textit{what-if} statement: if $p$ were true, then $q$ would be true as well.

\citeauthor{lewis2013counterfactuals} suggests the following interpretation:

\begin{quote}
    \textit{``If kangaroos had no tails, they would topple over''} seems to me to mean something like this: in any possible state of affairs in which kangaroos have no tails, and which resembles our actual state of affairs as much as kangaroos having no tails permits it to, the kangaroos topple over.
\end{quote}

Motivated by this interpretation, we wish to model possible ``states of affairs'' and their relationships as vectors in the latent space of a generative adversarial neural network.
Concretely, suppose:
\begin{itemize}
    \item The \textit{state of affairs} can be encoded as a vector $\mathbf{z \in \textbf{R}^n}$
    \item The notion of \textit{resemblance} between two states corresponds to a metric $\mathbf{||z_0 - z^*||}$
    \item There exists an indicator function $\mathbf{C_p(z)}$ that outputs 1 if $p$ is true given $z$.
\end{itemize}

Given an actual state $z_0$ and logical statements $p$ and $q$, finding the state of affairs in which $p$ is true that resembles $z_0$ as much as possible can be posed as a numerical optimization problem:

\begin{align*}
    \text{minimize} &&
    ||z_0 - z^*||_2 \\
    \text{subject to} &&
    C_p(z^*) = 1
\end{align*}

We treat $C_p: \mathbf{R}^n \rightarrow \{0, 1\}$ as an indicator function with the value $1$ if $p$ is true.
Given the optimal $z^*$, the truth value of the original counterfactual conditional can be determined:

$$
p \  \counterfactual q \Longleftrightarrow C_q(z^*) = 1
$$


For example, let $z$ be the latent representation of an Atari frame concatenated with predicted memory and $\pi$.
%Given an image of a random digit and its latent representation $z_0$, our formulation of counterfactual image generation can be used to answer the question ``what would this image look like if this were a digit `3'?'', where $p$ is ``being digit 3''.
Given a sequence of Atari frames and its latent representation $z_0$, our formulation of counterfactual image generation can be used to answer the question ``what would this frame look like if the agent were to take a different action $a'$ '', where $p$ is ``take action $a'$ ''.

%TODO: add figures: there will be 4 states total, 2 for pong and 2 for space invaders
In Figure 2, we show images of the current frame (left column), the action taken by $\pi$, and the counterfactual images generated by optimizing them toward other actions for the games Space Invaders and Pong.
We can see that by starting from different sequences, the generated counterfactual images are still relatively the same as the original frame, but differ significantly from one another on the same action $a'$. 
%This shows how we satisfy the minimization constraint

Optimization in the latent space is capable of producing examples that lie outside of the distribution of possible classes, but nonetheless remain within a larger distribution within pixel space consisting of plausible images.
The counterfactual image optimization connects to the concept of adversarial image generation explored in \cite{goodfellow2014explaining} and \cite{moosavi2016deepfool}.
%Gradient descent on the classification objective regularized by an L2 distance metric produces an output that is close in content to the original, perturbed just enough to change its class identity.
Optimization in pixel space produces adversarial examples, and while the counterfactual optimization is constrained to a manifold of realistic images learned by the generative model, the states produced may not be reachable by normal gameplay.

%TODO:  be more explicit about how counterfactuals until probability of C(a') = 1 generates adversarial examples... Question: does this occur with a GAN model?

\subsection{Generating Counterfactuals}
Our goal is to use counterfactual image generation to generate synthetic images that closely resemble real states of the game environment, but lie on the other side of the action decision boundary between the agent taking action $a$ and the agent taking a different action $a'$.
This can be formulated as follows:

%How to appropriately formulate the fact the synthetic memory is used as input?
\begin{align*}
    \text{minimize} &&
    ||A(s) - z^*||_2 \\
    \text{subject to} &&
    \arg \max_{a\epsilon Actions} \pi(z^*)) = a'
\end{align*}
where $s$ is the given initial real.

We will use the agent $\pi$ to determine when a different action should be taken on the given state. We deem a different action to be taken when the agents' probability of taking action $a'$ is the highest of all actions. 

Specifically, we formulate the following objective for counterfactual generation:

% This is what I have referred to as the "counterfactual optimization"
%How do I convert this pytorch code into math?
%loss = F.nll_loss(logp, target_action)
%da_dz = autograd.grad(loss, z, loss)[0]
%z = z - da_dz * speed

\begin{equation}
z^* = \min_{z}
||z - A(s)||_2^2
+
\log \left(1 - P(a'|\pi(z)) \right)
\end{equation}

Here $\pi(z)$ is the list of probabilities of the Agent for taking discrete action $a$ on the counterfactual state $z$.
The second term of the objective is the negative log-likelihood of taking action $a'$.
By minimizing this term, we aim to increase the probability of taking action $a'$ and reduce the probability of taking all other actions.

To generate a counterfactual image, we select an input state $s$ from a game sequence.
We encode the image to a latent point $z = A(s)$, then minimize equation (3) through gradient descent for a fixed number of steps, or until the highest probability action is $a'$, to find $z^*$, then decode the latent point to generate the counterfactual image $G(E(s);z^*)$.
This counterfactual image is the closest state representation of the input $s$ while still having the agent take a different action (see fig \ref{fig:cf_qbert} for an example).


\begin{figure}[t]
\begin{center}
    \includegraphics[width=\linewidth]{pong_moveup.png}
\end{center}
\caption{\textbf{Left:} The original state of Pong (arrow indicating ball velocity), where the agent would stay still. \textbf{Right:} The state where the an agent would take the "Move Up" action. The agent is trying to line up a "kill shot" where the ball hits the corner of the paddle. If the ball where higher, then the agent would need to start moving up in order to reach this "kill shot". }
\end{figure}

\begin{figure}[t]
\begin{center}
    \includegraphics[width=\linewidth]{qbert_cfexample_4_.png}
\end{center}
\caption{\textbf{Left}: The original state of Qbert where the agent would take the "jump up and right" action. \textbf{Right}: The state where the agent would take the "jump down and right" action. The agent would only jump closer to the enemy if it means progressing through the level. }
\label{fig:cf_qbert}
\end{figure}

\begin{figure*}[t]
\begin{center}
    \includegraphics[width=\linewidth]{qbert_imitation_agent_lowest_entropy.png}
\end{center}
\caption{\textbf{Top}: The original state of Qbert. \textbf{Bottom}: The state where the non-robust agent would take a different action. Notice how almost all of the states are not realistic: either the agent had landed on places that were impossible to reach, or the frame must have non-existent artifacts.}
\end{figure*}

